Quark sector of Coulomb gauge Quantum Chromodynamics

The quark sector of Coulomb gauge quantum chromodynamics is considered within the functional integral approach. The quark contributions to the Dyson-Schwinger equations are derived and one-loop perturbative results for the two-point functions are presented. The problem of confinement is addressed in the heavy quark limit, by rewriting the generating functional of quantum chromodynamics in terms of a heavy quark mass expansion. By restricting to leading order in this expansion and considering only the two-point functions of the Yang-Mills sector, the rainbow-ladder approximation to the gap and Bethe-Salpeter equations is shown to be exact. Analytic nonperturbative solutions to the Bethe-Salpeter equation for quark-antiquark bound states and Faddeev equation for three-quark bound states, in the case of equal quark separations, are presented. The quark-antiquark and three-quark confining potentials are derived and a direct connection between the temporal gluon propagator and the corresponding string tensions is found. It is shown that only color singlet of quark-antiquark (meson) and qqq (baryon) states are physically allowed. Moreover, the four-point Green's functions, in both quark-antiquark and diquark channels, are explicitly derived. It is found that the corresponding poles relate to the bound state energy of the heavy quark systems, and a natural separation between physical and unphysical poles in the Green's functions emerges.

==> intro.tex <==


\chapter{Introduction}
\label{chap1} 

{\bf QCD explicit}

Quantum Chromodynamics (QCD) is the theory of strong interactions between
the fundamental constituents, the quarks and gluons
\cite{Peskin:1995ev, Itzykson:1980rh,Muta:1998vi,Ryder:1985wq}.
    
A deep understanding of QCD requires a whole toolbox
of theoretical methods. In addition to analytical perturbative methods
for weak coupling and nummerical lattice gauge theory for arbitrary
couplings,  the cannonical approach \cite{Abers:1973qs} and the
functional methods 
\cite{Itzykson:1980rh}
 aim to bridge the gap, since they are
not restricted to weak coupling and can still be treated
analytically. 
In the canonical
approach, the Yang-Mills Schr\"odinger equation
was solved variationally for the vacuum state using Gaussian type
ans\"atze for the wave functional,
%. Minimizing the energy density
%results in a coupled set of of \DS equations which have been solved
%analytically in the infrared and numerically in the whole momentum
%regime,
 leading to clear signals of confinement \cite{Reinhardt:2004mm, Feuchter:2004mk}.
 %However, in spite of
%this success, one should bear in mind that an ansatz for the
%wave-functional is always required and so the approach does not a
%priori provide a systematic expansion or truncation scheme as, for
%example, the loop expansion used in the common \DS approach.
The functional methods most commonly used are 
the renormalization group equations (see \cite{Gies:2006wv} for a
review) and the \DS equations
\cite{Dyson:1949ha, Schwinger:1951ex,  Schwinger:1951hq}.
 These are esentially the equations of motion for the QCD Green's
functions, analogous to Euler-Lagrange equation in classical field theory.
In this work we will concentrate on the study of the \DS equations
for the quark sector of  Coulomb gauge QCD, 
%The idea is to express the $n$-point Green's functions in
%terms of the elementary two point functions of the theory, i.e. the
%quark, ghost and gluon propagators.
which has the advantage that it is ''physical'', in the sense
that the number of dynamical variables reduces to the number of the
physical degrees of freedom \cite{Zwanziger:1998ez} and moreover,  the Gribov-Zwanziger confinement
scenario \cite{Zwanziger:1998ez, Gribov:1977wm} becomes particularly relevant in Coulomb gauge. 
%In this
%picture, the temporal component of the gluon propagator provides the
%long-range confinimg force while the spatial components are supressed
%in the infrared. 

....

In this work we are concerned with the phenomena which occur at both
large and small momentum transfers of the quarks. At large momentum
transfer, the physical phenomena are good described by the
perturbation theory. In the small coupling limit, one can calculate
the quark mass and show that the renormalzed mass is physical...

The other phenomenon that we are concerned with is the confinement
phenomenon. This can not be accounted for in perturbation theory --
strong QCD

Heavy quarks

Framework: DS equations

compare with Landau gauge and the results of HQET (potential models)
